Neural Control Variates

We propose neural control variates (NCV) for unbiased variance reduction in parametric Monte Carlo integration. So far, the core challenge of applying the method of control variates has been finding a good approximation of the integrand that is cheap to integrate. We show that a set of neural networks can face that challenge: a normalizing flow that approximates the shape of the integrand and another neural network that infers the solution of the integral equation. We also propose to leverage a neural importance sampler to estimate the difference between the original integrand and the learned control variate. To optimize the resulting parametric estimator, we derive a theoretically optimal, variance-minimizing loss function, and propose an alternative, composite loss for stable online training in practice. When applied to light transport simulation, neural control variates are capable of matching the state-of-the-art performance of other unbiased approaches, while providing means to develop more performant, practical solutions. Specifically, we show that the learned light-field approximation is of sufficient quality for high-order bounces, allowing us to omit the error correction and thereby dramatically reduce the noise at the cost of negligible visible bias.

==> __latexindent_temp.tex <==

\section{Variance of CV Estimator}
\label{sec:variance-derivation}

We are interested in deriving the variance of the following estimator:
\begin{align}
    \MC{F} = \CV(\CVParams) + \frac{f(X,Z)}{\PdfMC(X,Z)}  - \frac{\cv(X;\cvParams)}{\PdfMC(X)} \,.
    \label{eq:mc-integrator-with-z-appendix}
\end{align}
To simplify the derivation, we subtract the constant $\CV(\CVParams)$ from both sides and proceed with the definition of variance:
\begin{align}
    \Variance\left[\MC{F} - \CV(\CVParams)\right] &= \Expectation\left[ \left({\MC{F} - \CV(\CVParams)}\right)^2 \right] - {\Expectation\left[ \MC{F} - \CV(\CVParams) \right]}^2
    \,.
    \label{eq:mc-variance-derivation-appendix}
\end{align}
Since $\Variance[X + c] = \Variance[X]$, the left-hand side simplifies to $\Variance\left[\MC{F}\right]$.
The expectation of the square can be expressed as the following double integral:
\begin{align}
    \Expectation\left[ \left({\MC{F} \!-\! \CV(\CVParams)}\right)^2 \right]
    \!&=
    \Expectation\left[ \left(
        \frac{f(X,Z)}{\PdfMC(X,Z)}  - \frac{\cv(X;\cvParams)}{\PdfMC(X)}
    \right)^2 \right] \nonumber\\
    &=\!\! \int_\Domain \! \int_\DomainZ \!\! \left( \frac{f(x,z)}{\PdfMC(x,z)} - \frac{\cv(x;\cvParams)}{\PdfMC(x)}\right)^2
     \PdfMC(x,z) \Diff{z}\!\Diff{x}
    \nonumber \\
    &=\!\! \int_\Domain \! \int_\DomainZ \!\! \left( \frac{f(x,z)}{\PdfMC(x)\PdfMC(z|x)} - \frac{\cv(x;\cvParams)}{\PdfMC(x)}\right)^2
     \!\PdfMC(x)\PdfMC(z|x) \Diff{z}\!\Diff{x}
    \nonumber \\
    &=\!\! \int_\Domain \! \int_\DomainZ \!\! \left( \frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams)\right)^2\frac{\PdfMC(z|x)}{\PdfMC(x)} \Diff{z}\!\Diff{x}
\label{eq:mc-expectation-of-square-appedix}
\end{align}
The squared expectation (second term in \autoref{eq:mc-variance-derivation-appendix}) simplifies to $\left(\Expectation\left[\MC{F}\right] - \CV(\CVParams) \right)^2 = \left(F - \CV(\CVParams) \right)^2$.
Putting all the terms together yields \autoref{eq:mc-variance-with-tail}.



\section{Variance Gradients}
\label{sec:variance-gradient-derivation}
We derive gradients for two estimators: 1) an estimator with a parametric CV and a \emph{fixed} sampler for estimating the difference integral, and 2) an estimator with parametric CV and a parametric, \emph{trainable} sampler (such as those proposed by \citet{mueller2019nis}).

\subsection{Trainable CV and Fixed Sampler}
For ease of notation, we split the variance function into two terms, $A$ and $B$:
\begin{align}
    \Variance\left[\MC{F}\right]
    &= \underbrace{\!\int_\Domain \!\int_\DomainZ \! \left( \frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams)\right)^2\frac{\PdfMC(z|x)}{\PdfMC(x)} \Diff{z}\!\Diff{x}}_{A}
    - \underbrace{(F - \CV(\CVParams))^2}_{B}.
\label{eq:mc-variance-with-tail-appendix}
\end{align}
The variance gradient $\nabla_{\cvParams} \Variance\left[\MC{F}\right] = \nabla_{\cvParams} A - \nabla_{\cvParams} B$ consists of the following:
\begin{align}
\nabla_{\cvParams}A
&= \nabla_{\cvParams}\!\int_\Domain \!\int_\DomainZ \! \left( \frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams)\right)^2\frac{\PdfMC(z|x)}{\PdfMC(x)} \Diff{z}\!\Diff{x}
\nonumber\\
&= \!\int_\Domain \!\int_\DomainZ \!\nabla_{\cvParams} \left( \frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams)\right)^2\frac{\PdfMC(z|x)}{\PdfMC(x)} \Diff{z}\!\Diff{x}
\nonumber\\
&= -2 \int_\Domain
\frac{ \int_\DomainZ f(x,z) - \cv(x;\cvParams) \PdfMC(z|x)  \Diff{z} }{\PdfMC(x)}
\nabla_{\cvParams} \cv(x;\cvParams)
\Diff{x}
\nonumber\\
&= -2 \int_\Domain
\frac{f(x) - \cv(x;\cvParams) }{\PdfMC(x)}
\nabla_{\cvParams} \cv(x;\cvParams)
\Diff{x}\,,
\\
\nonumber\\
\nabla_{\cvParams}B
&= \nabla_{\CVParams} \left(F - \CV(\CVParams)\right)^2
\nonumber\\
&= -2\, \left(F - \CV(\CVParams)\right) \,\nabla_{\CVParams} \CV(\CVParams)\,.
\label{eq:mc-variance-with-tail-appendix}
\end{align}
Putting the terms together:
\begin{align}
\nabla_{\cvParams} \Variance\left[\MC{F}\right] =
&-2 \int_\Domain
\frac{f(x) - \cv(x;\cvParams) }{\PdfMC(x)}
\nabla_{\cvParams} \cv(x;\cvParams)
\Diff{x}\\
&+2\, \left(F - \CV(\CVParams)\right) \,\nabla_{\CVParams} \CV(\CVParams)\,.
\end{align}

Since the gradient cannot be evaluated in closed form (due to the presence of integral $F$, which is unknown, and likely also because of the difference integral), we can estimate the two integrals using the following one-sample estimator:
\begin{align}
    \MC{\nabla_{\cvParams} \Variance\left[\MC{F}\right]} =
    &-2
    \frac{\MC{f(x)} - \cv(x;\cvParams) }{\PdfMC(x) \PdfVarEst(x)}
    \nabla_{\cvParams} \cv(x;\cvParams)
    \\
    &+2\, \left(\frac{\MC{f(x)}}{\PdfVarEst(x)} - \CV(\CVParams)\right) \,\nabla_{\CVParams} \CV(\CVParams)\,.
\end{align}
The above estimator is unbiased as long as $\MC{f(x)}$ is unbiased: the other terms merely scale and offset $\MC{f(x)}$ preserving the zero-mean distribution of the stochastic error.



\subsection{Trainable CV and Trainable Sampler}
We now consider the case of a parametric, optimizable probability density $\PdfMC(x;\pdfParams)$.


\begin{align}
    \nabla_{\Params}A
    &= \nabla_{\Params}\!\int_\Domain \!\int_\DomainZ \! \left( \frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams)\right)^2\frac{\PdfMC(z|x)}{\PdfMC(x;\pdfParams)} \Diff{z}\!\Diff{x}
    \nonumber\\
    &=
    \int_\Domain \int_\DomainZ
    - \frac{\PdfMC(z|x) \left(\frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams)\right)
    \left(
        \left(\frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams) \right)  \nabla_{\pdfParams}\PdfMC(x;\pdfParams)
        +
        2 \PdfMC(x;\pdfParams) \nabla_{\cvParams} \cv(x, \cvParams)
    \right)
    }{ \PdfMC(x;\pdfParams)^2 }
    \label{eq:mc-variance-with-tail-appendix}
    \end{align}


\newpage
\onecolumn
I'm curious how you derived the gradient in the case of NCV+NIS.
Let's just focus on the following term of variance:
\begin{align}
    \int_\Domain  \frac{ (f - \cv(\cvParams))^2}{\PdfMC(\pdfParams)} \Diff{x}
\end{align}
Denoting $\Params = \cvParams \cup \pdfParams$, we can derive the gradient using the product rule:
\begin{align}
    \nabla_{\Params}  \int_\Domain  \frac{ (f - \cv(\cvParams))^2}{\PdfMC(\pdfParams)} \Diff{x}
    &=
    \int_\Domain \nabla_{\Params}  \left( (f - \cv(\cvParams))^2 \cdot \frac{1}{\PdfMC(\pdfParams)} \right)  \Diff{x}
    \\
    &= \int_\Domain \left(-2 (f - \cv(\cvParams)) \nabla_{\cvParams} \cv(\cvParams)   \frac{1}{\PdfMC(\pdfParams)} \right)
    +
    \left(\right)
    \\
\end{align}

==> all-components-figure.tex <==
\setlength{\fboxrule}{1pt}%
\setlength{\insetvsep}{20pt}%
\setlength{\tabcolsep}{1pt}%
\renewcommand{\arraystretch}{0.75}%
\small%
\hspace*{-3mm}%
\begin{tabular}{rccccc}
& CV Integral $\CV(\pos, \diro; \CVParams)$ & Coefficient $\cvCoef(\pos, \diro; \cvCoefParams)$ & Selection Probability $\selectionProb(\pos, \diro; \selectionProbParams)$ & CV $\cv(\pos, \diro, \diri; \cvParams)$ & PDF $\PdfMC(\pos, \diro, \diri; \pdfParams)$ \\
    \multirow[t]{2}{*}{\small\rotatebox{90}{\hspace{0.70cm}\Bathroom{}}} & 
    \multirow[t]{2}{*}{\begin{overpic}[width=0.237\textwidth]{images/fig-all-components/cam-0-bathroom/target-control-variate-36.jpg}\put(45.364583333333336,2.265625){\makebox(0,0){\tikz\draw[red,fill=red] (0,0) circle (0.0023699999999999997\textwidth);}}\end{overpic}} & \multirow[t]{2}{*}{\begin{overpic}[width=0.237\textwidth]{images/fig-all-components/cam-0-bathroom/target-alpha-36.jpg}\put(45.364583333333336,2.265625){\makebox(0,0){\tikz\draw[red,fill=red] (0,0) circle (0.0023699999999999997\textwidth);}}\end{overpic}} & \multirow[t]{2}{*}{\begin{overpic}[width=0.237\textwidth]{images/fig-all-components/cam-0-bathroom/target-selection-prob-36.jpg}\put(45.364583333333336,2.265625){\makebox(0,0){\tikz\draw[red,fill=red] (0,0) circle (0.0023699999999999997\textwidth);}}\end{overpic}} & \color{red}\fbox{\includegraphics[width=0.13064625\textwidth]{images/fig-all-components/cam-0-bathroom/target-dist-0-cv-36.jpg}} & \color{red}\fbox{\includegraphics[width=0.13064625\textwidth]{images/fig-all-components/cam-0-bathroom/target-dist-0-pdf-36.jpg}} \\
    \multirow[t]{2}{*}{\small\rotatebox{90}{\hspace{0.70cm}\Bedroom{}}} & 
    \multirow[t]{2}{*}{\begin{overpic}[width=0.237\textwidth]{images/fig-all-components/cam-0-bedroom/target-control-variate-36.jpg}\put(49.947916666666664,6.927083333333334){\makebox(0,0){\tikz\draw[red,fill=red] (0,0) circle (0.0023699999999999997\textwidth);}}\end{overpic}} & \multirow[t]{2}{*}{\begin{overpic}[width=0.237\textwidth]{images/fig-all-components/cam-0-bedroom/target-alpha-36.jpg}\put(49.947916666666664,6.927083333333334){\makebox(0,0){\tikz\draw[red,fill=red] (0,0) circle (0.0023699999999999997\textwidth);}}\end{overpic}} & \multirow[t]{2}{*}{\begin{overpic}[width=0.237\textwidth]{images/fig-all-components/cam-0-bedroom/target-selection-prob-36.jpg}\put(49.947916666666664,6.927083333333334){\makebox(0,0){\tikz\draw[red,fill=red] (0,0) circle (0.0023699999999999997\textwidth);}}\end{overpic}} & \color{red}\fbox{\includegraphics[width=0.13064625\textwidth]{images/fig-all-components/cam-0-bedroom/target-dist-0-cv-36.jpg}} & \color{red}\fbox{\includegraphics[width=0.13064625\textwidth]{images/fig-all-components/cam-0-bedroom/target-dist-0-pdf-36.jpg}} \\
\end{tabular}


==> nis-cv-scale-figure.tex <==
\setlength{\fboxrule}{10pt}%
\setlength{\insetvsep}{20pt}%
\setlength{\tabcolsep}{-1pt}%
\renewcommand{\arraystretch}{1}%
\small%
\hspace*{-2mm}%
\begin{tabular}{rcccc}
  {} & {} & w/ NIS & w/ NCV & Reference \\
    \setInset{A}{red}{820}{580}{140}{180}%
    \setInset{B}{orange}{1130}{580}{140}{180}%
    \rotatebox{90}{\hspace{-2.00cm}\VeachDoor{}}\hspace{0.14cm} &
    \addBeautyCrop{images/fig-references/veach-door-reference.jpg}{0.25}{1920}{1080}{300}{0}{1520}{1080} &
    \addInsets{images/fig-nis-cv-scale/veach-door-job6139.jpg} &
    \addInsets{images/fig-nis-cv-scale/veach-door-job5289.jpg} &
    \addInsets{images/fig-references/veach-door-reference.jpg} \\
  & \multicolumn{1}{r}{MAPE:} & 0.069 & \textbf{0.030} \\
\end{tabular}


==> results-light-field-figure.tex <==
\setlength{\fboxrule}{1pt}%
\setlength{\insetvsep}{20pt}%
\setlength{\tabcolsep}{1pt}%
\renewcommand{\arraystretch}{0.75}%
\small%
\hspace*{-3mm}%
\begin{tabular}{rccl}
& CV Integral at First Non-Specular Vertex & & \\
    & & \color{red}\fbox{\includegraphics[width=0.10006009615384616\textwidth]{images/fig-light-field/cam-0-bathroom/target-dist-0-cv-36.jpg}} & \rotatebox{90}{\hspace{0.7cm}CV}\\
    \multirow[t]{2}{*}{\rotatebox{90}{\hspace{1.30cm}\Bathroom{}}} & 
    \multirow[t]{2}{*}{\begin{overpic}[width=0.37\textwidth]{images/fig-light-field/cam-0-bathroom/target-control-variate-36.jpg}\put(45.364583333333336,2.265625){\makebox(0,0){\tikz\draw[red,fill=red] (0,0) circle (0.0037\textwidth);}}\end{overpic}} & 
    \color{red}\fbox{\includegraphics[width=0.10006009615384616\textwidth]{images/fig-light-field/cam-0-bathroom/target-dist-0-pdf-36.jpg}} & \rotatebox{90}{\hspace{0.6cm}PDF}\\
    & & \color{red}\fbox{\includegraphics[width=0.10006009615384616\textwidth]{images/fig-light-field/cam-0-bedroom/target-dist-0-cv-36.jpg}} & \rotatebox{90}{\hspace{0.7cm}CV}\\
    \multirow[t]{2}{*}{\rotatebox{90}{\hspace{1.30cm}\Bedroom{}}} & 
    \multirow[t]{2}{*}{\begin{overpic}[width=0.37\textwidth]{images/fig-light-field/cam-0-bedroom/target-control-variate-36.jpg}\put(49.947916666666664,6.927083333333334){\makebox(0,0){\tikz\draw[red,fill=red] (0,0) circle (0.0037\textwidth);}}\end{overpic}} & 
    \color{red}\fbox{\includegraphics[width=0.10006009615384616\textwidth]{images/fig-light-field/cam-0-bedroom/target-dist-0-pdf-36.jpg}} & \rotatebox{90}{\hspace{0.6cm}PDF}\\
    & & \color{red}\fbox{\includegraphics[width=0.10006009615384616\textwidth]{images/fig-light-field/cam-0-spaceship/target-dist-0-cv-36.jpg}} & \rotatebox{90}{\hspace{0.7cm}CV}\\
    \multirow[t]{2}{*}{\rotatebox{90}{\hspace{1.30cm}\Spaceship{}}} & 
    \multirow[t]{2}{*}{\begin{overpic}[width=0.37\textwidth]{images/fig-light-field/cam-0-spaceship/target-control-variate-36.jpg}\put(52.84739583333333,18.958333333333332){\makebox(0,0){\tikz\draw[red,fill=red] (0,0) circle (0.0037\textwidth);}}\end{overpic}} & 
    \color{red}\fbox{\includegraphics[width=0.10006009615384616\textwidth]{images/fig-light-field/cam-0-spaceship/target-dist-0-pdf-36.jpg}} & \rotatebox{90}{\hspace{0.6cm}PDF}\\
\end{tabular}


==> results-metrics-table-time.tex <==
\small
\rowcolors{2}{white}{gray!8}
\setlength{\tabcolsep}{6.33pt}
\begin{tabular*}{\textwidth}{rccccccc}
  \toprule
  {} & \multicolumn{5}{c}{Unbiased} & \multicolumn{2}{c}{Biased} \\
  \cmidrule(lr){2-6}
  \cmidrule(lr){7-8}
  \rowcolor{white}
  {} & {} & \citep{mueller19guiding} & \citep{mueller2019nis} & \multicolumn{4}{c}{Ours} \\
  \cmidrule(lr){3-3}
  \cmidrule(lr){4-4}
  \cmidrule(lr){5-8}
  \rowcolor{white}
  {} & PT & PPG & NIS & NIS++ & NCV & NCV + heuristic & CV Integral \\
  \midrule
  \small{\Artroom{}} & \small{\makebox[0.6cm]{1.393} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.108} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.079} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.062} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.056}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.044}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.091} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\Bathroom{}} & \small{\makebox[0.6cm]{0.112} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.073} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.041} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.037} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.030}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.017}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.023} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\Bedroom{}} & \small{\makebox[0.6cm]{0.064} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.035} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.031} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.031} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.026}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.020}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.035} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\Bookshelf{}} & \small{\makebox[0.6cm]{0.658} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.045} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.054} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.047} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.030}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.025}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.080} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\Bottle{}} & \small{\makebox[0.6cm]{0.848} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.088} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.084} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.062} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.056}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.046}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.163} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\CornellBox{}} & \small{\makebox[0.6cm]{0.035} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.009} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.009} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.009} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.005}} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} & \small{\makebox[0.6cm]{\textbf{0.006}} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} & \small{\makebox[0.6cm]{0.020} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} \\
  \small{\CrytekSponza{}} & \small{\makebox[0.6cm]{1.340} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.056} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.065} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.060} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.051}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.048}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.234} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\GlossyKitchen{}} & \small{\makebox[0.6cm]{1.450} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.071} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.075} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.049} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.045}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.031}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.114} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\CountryKitchen{}} & \small{\makebox[0.6cm]{0.696} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.068} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.073} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.066} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.059}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.046}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.067} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\Necklace{}} & \small{\makebox[0.6cm]{0.289} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.057} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.038} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.033} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} & \small{\makebox[0.6cm]{\textbf{0.031}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.030}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.159} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\SwimmingPool{}} & \small{\makebox[0.6cm]{0.451} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.035} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.040} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.034} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.031}} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} & \small{\makebox[0.6cm]{\textbf{0.028}} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} & \small{\makebox[0.6cm]{0.076} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} \\
  \small{\Spaceship{}} & \small{\makebox[0.6cm]{0.017} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.009} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.009} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.008} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.006}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.007}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.027} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\SpectralBox{}} & \small{\makebox[0.6cm]{0.030} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.014} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.017} \, \makebox[0.6cm]{\textcolor{gray}{2.2h}}} & \small{\makebox[0.6cm]{0.015} \, \makebox[0.6cm]{\textcolor{gray}{2.3h}}} & \small{\makebox[0.6cm]{\textbf{0.009}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.008}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.019} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\Sponza{}} & \small{\makebox[0.6cm]{1.614} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.060} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.049} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.040}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.042} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} & \small{\makebox[0.6cm]{\textbf{0.022}} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} & \small{\makebox[0.6cm]{0.066} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} \\
  \small{\Staircase{}} & \small{\makebox[0.6cm]{0.137} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.029} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.023} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.022} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.019}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.015}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.036} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\Torus{}} & \small{\makebox[0.6cm]{0.214} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.021} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.020} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.018} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.015}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.014}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.014} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\VeachDoor{}} & \small{\makebox[0.6cm]{0.532} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.084} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.065} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.060} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.036}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{\textbf{0.024}} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.034} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} \\
  \small{\VeachLamp{}} & \small{\makebox[0.6cm]{0.532} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.069} \, \makebox[0.6cm]{\textcolor{gray}{2.0h}}} & \small{\makebox[0.6cm]{0.077} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} & \small{\makebox[0.6cm]{0.068} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} & \small{\makebox[0.6cm]{\textbf{0.039}} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} & \small{\makebox[0.6cm]{0.026} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} & \small{\makebox[0.6cm]{\textbf{0.022}} \, \makebox[0.6cm]{\textcolor{gray}{2.1h}}} \\
  \bottomrule
\end{tabular*}


==> results-metrics-table.tex <==
\small
\rowcolors{2}{white}{gray!8}
\setlength{\tabcolsep}{6.33pt}
\begin{tabular*}{\textwidth}{rccccccc}
  \toprule
  {} & \multicolumn{5}{c}{Unbiased} & \multicolumn{2}{c}{Biased} \\
  \cmidrule(lr){2-6}
  \cmidrule(lr){7-8}
  \rowcolor{white}
  {} & {} & \citep{mueller2017practical} & \citep{mueller2019nis} & \multicolumn{4}{c}{Ours} \\
  \cmidrule(lr){3-3}
  \cmidrule(lr){4-4}
  \cmidrule(lr){5-8}
  \rowcolor{white}
  {} & PT & PPG & NIS no decay & NIS & NCV & NCV & CV integral \\
  \midrule
  \small{\Artroom{}} & \small{\makebox[0.6cm]{1.393} \, \makebox[0.7cm]{\textcolor{gray}{1,756 spp}}} & \small{\makebox[0.6cm]{0.108} \, \makebox[0.7cm]{\textcolor{gray}{2,998 spp}}} & \small{\makebox[0.6cm]{0.084} \, \makebox[0.7cm]{\textcolor{gray}{1,150 spp}}} & \small{\makebox[0.6cm]{0.065} \, \makebox[0.7cm]{\textcolor{gray}{1,181 spp}}} & \small{\makebox[0.6cm]{nan} \, \makebox[0.7cm]{\textcolor{gray}{7 spp}}} & \small{\makebox[0.6cm]{nan} \, \makebox[0.7cm]{\textcolor{gray}{7 spp}}} & \small{\makebox[0.6cm]{nan} \, \makebox[0.7cm]{\textcolor{gray}{7 spp}}} \\
  \small{\Bathroom{}} & \small{\makebox[0.6cm]{0.112} \, \makebox[0.7cm]{\textcolor{gray}{1,785 spp}}} & \small{\makebox[0.6cm]{0.106} \, \makebox[0.7cm]{\textcolor{gray}{1,023 spp}}} & \small{\makebox[0.6cm]{0.041} \, \makebox[0.7cm]{\textcolor{gray}{667 spp}}} & \small{\makebox[0.6cm]{0.038} \, \makebox[0.7cm]{\textcolor{gray}{648 spp}}} & \small{\makebox[0.6cm]{\textbf{0.033}} \, \makebox[0.7cm]{\textcolor{gray}{676 spp}}} & \small{\makebox[0.6cm]{\textbf{0.017}} \, \makebox[0.7cm]{\textcolor{gray}{676 spp}}} & \small{\makebox[0.6cm]{0.024} \, \makebox[0.7cm]{\textcolor{gray}{676 spp}}} \\
  \small{\Bedroom{}} & \small{\makebox[0.6cm]{0.064} \, \makebox[0.7cm]{\textcolor{gray}{1,727 spp}}} & \small{\makebox[0.6cm]{0.035} \, \makebox[0.7cm]{\textcolor{gray}{2,187 spp}}} & \small{\makebox[0.6cm]{0.034} \, \makebox[0.7cm]{\textcolor{gray}{612 spp}}} & \small{\makebox[0.6cm]{0.032} \, \makebox[0.7cm]{\textcolor{gray}{621 spp}}} & \small{\makebox[0.6cm]{\textbf{0.029}} \, \makebox[0.7cm]{\textcolor{gray}{636 spp}}} & \small{\makebox[0.6cm]{\textbf{0.022}} \, \makebox[0.7cm]{\textcolor{gray}{636 spp}}} & \small{\makebox[0.6cm]{0.036} \, \makebox[0.7cm]{\textcolor{gray}{636 spp}}} \\
  \small{\Bookshelf{}} & \small{\makebox[0.6cm]{0.658} \, \makebox[0.7cm]{\textcolor{gray}{2,113 spp}}} & \small{\makebox[0.6cm]{\textbf{0.045}} \, \makebox[0.7cm]{\textcolor{gray}{2,749 spp}}} & \small{\makebox[0.6cm]{0.059} \, \makebox[0.7cm]{\textcolor{gray}{868 spp}}} & \small{\makebox[0.6cm]{0.050} \, \makebox[0.7cm]{\textcolor{gray}{895 spp}}} & \small{\makebox[0.6cm]{0.047} \, \makebox[0.7cm]{\textcolor{gray}{882 spp}}} & \small{\makebox[0.6cm]{\textbf{0.032}} \, \makebox[0.7cm]{\textcolor{gray}{882 spp}}} & \small{\makebox[0.6cm]{0.088} \, \makebox[0.7cm]{\textcolor{gray}{882 spp}}} \\
  \small{\Bottle{}} & \small{\makebox[0.6cm]{0.848} \, \makebox[0.7cm]{\textcolor{gray}{2,110 spp}}} & \small{\makebox[0.6cm]{0.088} \, \makebox[0.7cm]{\textcolor{gray}{3,612 spp}}} & \small{\makebox[0.6cm]{0.089} \, \makebox[0.7cm]{\textcolor{gray}{1,190 spp}}} & \small{\makebox[0.6cm]{\textbf{0.065}} \, \makebox[0.7cm]{\textcolor{gray}{1,313 spp}}} & \small{\makebox[0.6cm]{0.427} \, \makebox[0.7cm]{\textcolor{gray}{63 spp}}} & \small{\makebox[0.6cm]{\textbf{0.231}} \, \makebox[0.7cm]{\textcolor{gray}{63 spp}}} & \small{\makebox[0.6cm]{0.413} \, \makebox[0.7cm]{\textcolor{gray}{63 spp}}} \\
  \small{\CornellBox{}} & \small{\makebox[0.6cm]{0.035} \, \makebox[0.7cm]{\textcolor{gray}{8,614 spp}}} & \small{\makebox[0.6cm]{0.009} \, \makebox[0.7cm]{\textcolor{gray}{3,873 spp}}} & \small{\makebox[0.6cm]{0.009} \, \makebox[0.7cm]{\textcolor{gray}{870 spp}}} & \small{\makebox[0.6cm]{0.008} \, \makebox[0.7cm]{\textcolor{gray}{883 spp}}} & \small{\makebox[0.6cm]{\textbf{0.006}} \, \makebox[0.7cm]{\textcolor{gray}{1,156 spp}}} & \small{\makebox[0.6cm]{\textbf{0.006}} \, \makebox[0.7cm]{\textcolor{gray}{1,156 spp}}} & \small{\makebox[0.6cm]{0.020} \, \makebox[0.7cm]{\textcolor{gray}{1,156 spp}}} \\
  \small{\CrytekSponza{}} & \small{\makebox[0.6cm]{1.340} \, \makebox[0.7cm]{\textcolor{gray}{1,518 spp}}} & \small{\makebox[0.6cm]{\textbf{0.056}} \, \makebox[0.7cm]{\textcolor{gray}{2,417 spp}}} & \small{\makebox[0.6cm]{0.066} \, \makebox[0.7cm]{\textcolor{gray}{558 spp}}} & \small{\makebox[0.6cm]{0.058} \, \makebox[0.7cm]{\textcolor{gray}{532 spp}}} & \small{\makebox[0.6cm]{0.059} \, \makebox[0.7cm]{\textcolor{gray}{650 spp}}} & \small{\makebox[0.6cm]{\textbf{0.046}} \, \makebox[0.7cm]{\textcolor{gray}{650 spp}}} & \small{\makebox[0.6cm]{0.209} \, \makebox[0.7cm]{\textcolor{gray}{650 spp}}} \\
  \small{\GlossyKitchen{}} & \small{\makebox[0.6cm]{1.450} \, \makebox[0.7cm]{\textcolor{gray}{2,092 spp}}} & \small{\makebox[0.6cm]{0.071} \, \makebox[0.7cm]{\textcolor{gray}{2,391 spp}}} & \small{\makebox[0.6cm]{0.074} \, \makebox[0.7cm]{\textcolor{gray}{811 spp}}} & \small{\makebox[0.6cm]{0.063} \, \makebox[0.7cm]{\textcolor{gray}{841 spp}}} & \small{\makebox[0.6cm]{\textbf{0.059}} \, \makebox[0.7cm]{\textcolor{gray}{806 spp}}} & \small{\makebox[0.6cm]{\textbf{0.046}} \, \makebox[0.7cm]{\textcolor{gray}{806 spp}}} & \small{\makebox[0.6cm]{0.148} \, \makebox[0.7cm]{\textcolor{gray}{806 spp}}} \\
  \small{\CountryKitchen{}} & \small{\makebox[0.6cm]{0.696} \, \makebox[0.7cm]{\textcolor{gray}{2,070 spp}}} & \small{\makebox[0.6cm]{0.068} \, \makebox[0.7cm]{\textcolor{gray}{3,013 spp}}} & \small{\makebox[0.6cm]{0.074} \, \makebox[0.7cm]{\textcolor{gray}{946 spp}}} & \small{\makebox[0.6cm]{0.071} \, \makebox[0.7cm]{\textcolor{gray}{930 spp}}} & \small{\makebox[0.6cm]{\textbf{0.067}} \, \makebox[0.7cm]{\textcolor{gray}{912 spp}}} & \small{\makebox[0.6cm]{\textbf{0.048}} \, \makebox[0.7cm]{\textcolor{gray}{912 spp}}} & \small{\makebox[0.6cm]{0.077} \, \makebox[0.7cm]{\textcolor{gray}{912 spp}}} \\
  \small{\Necklace{}} & \small{\makebox[0.6cm]{0.289} \, \makebox[0.7cm]{\textcolor{gray}{10,280 spp}}} & \small{\makebox[0.6cm]{0.057} \, \makebox[0.7cm]{\textcolor{gray}{9,449 spp}}} & \small{\makebox[0.6cm]{0.041} \, \makebox[0.7cm]{\textcolor{gray}{2,710 spp}}} & \small{\makebox[0.6cm]{\textbf{0.035}} \, \makebox[0.7cm]{\textcolor{gray}{2,721 spp}}} & \small{\makebox[0.6cm]{0.036} \, \makebox[0.7cm]{\textcolor{gray}{2,615 spp}}} & \small{\makebox[0.6cm]{\textbf{0.033}} \, \makebox[0.7cm]{\textcolor{gray}{2,615 spp}}} & \small{\makebox[0.6cm]{0.139} \, \makebox[0.7cm]{\textcolor{gray}{2,615 spp}}} \\
  \small{\SwimmingPool{}} & \small{\makebox[0.6cm]{0.451} \, \makebox[0.7cm]{\textcolor{gray}{4,271 spp}}} & \small{-} & \small{\makebox[0.6cm]{0.042} \, \makebox[0.7cm]{\textcolor{gray}{1,868 spp}}} & \small{\makebox[0.6cm]{\textbf{0.035}} \, \makebox[0.7cm]{\textcolor{gray}{1,908 spp}}} & \small{\makebox[0.6cm]{0.036} \, \makebox[0.7cm]{\textcolor{gray}{1,805 spp}}} & \small{\makebox[0.6cm]{\textbf{0.032}} \, \makebox[0.7cm]{\textcolor{gray}{1,805 spp}}} & \small{\makebox[0.6cm]{0.095} \, \makebox[0.7cm]{\textcolor{gray}{1,805 spp}}} \\
  \small{\Spaceship{}} & \small{\makebox[0.6cm]{0.017} \, \makebox[0.7cm]{\textcolor{gray}{6,489 spp}}} & \small{\makebox[0.6cm]{0.009} \, \makebox[0.7cm]{\textcolor{gray}{7,529 spp}}} & \small{\makebox[0.6cm]{0.009} \, \makebox[0.7cm]{\textcolor{gray}{2,454 spp}}} & \small{\makebox[0.6cm]{0.009} \, \makebox[0.7cm]{\textcolor{gray}{2,563 spp}}} & \small{\makebox[0.6cm]{\textbf{0.009}} \, \makebox[0.7cm]{\textcolor{gray}{2,244 spp}}} & \small{\makebox[0.6cm]{\textbf{0.008}} \, \makebox[0.7cm]{\textcolor{gray}{2,244 spp}}} & \small{\makebox[0.6cm]{0.030} \, \makebox[0.7cm]{\textcolor{gray}{2,244 spp}}} \\
  \small{\SpectralBox{}} & \small{\makebox[0.6cm]{0.030} \, \makebox[0.7cm]{\textcolor{gray}{9,563 spp}}} & \small{\makebox[0.6cm]{0.014} \, \makebox[0.7cm]{\textcolor{gray}{4,348 spp}}} & \small{\makebox[0.6cm]{0.017} \, \makebox[0.7cm]{\textcolor{gray}{930 spp}}} & \small{\makebox[0.6cm]{0.016} \, \makebox[0.7cm]{\textcolor{gray}{951 spp}}} & \small{\makebox[0.6cm]{\textbf{0.010}} \, \makebox[0.7cm]{\textcolor{gray}{1,199 spp}}} & \small{\makebox[0.6cm]{\textbf{0.009}} \, \makebox[0.7cm]{\textcolor{gray}{1,199 spp}}} & \small{\makebox[0.6cm]{0.019} \, \makebox[0.7cm]{\textcolor{gray}{1,199 spp}}} \\
  \small{\Sponza{}} & \small{\makebox[0.6cm]{1.614} \, \makebox[0.7cm]{\textcolor{gray}{1,904 spp}}} & \small{\makebox[0.6cm]{0.060} \, \makebox[0.7cm]{\textcolor{gray}{3,007 spp}}} & \small{\makebox[0.6cm]{0.050} \, \makebox[0.7cm]{\textcolor{gray}{556 spp}}} & \small{\makebox[0.6cm]{\textbf{0.042}} \, \makebox[0.7cm]{\textcolor{gray}{553 spp}}} & \small{\makebox[0.6cm]{0.044} \, \makebox[0.7cm]{\textcolor{gray}{708 spp}}} & \small{\makebox[0.6cm]{\textbf{0.024}} \, \makebox[0.7cm]{\textcolor{gray}{708 spp}}} & \small{\makebox[0.6cm]{0.062} \, \makebox[0.7cm]{\textcolor{gray}{708 spp}}} \\
  \small{\Staircase{}} & \small{\makebox[0.6cm]{0.137} \, \makebox[0.7cm]{\textcolor{gray}{1,458 spp}}} & \small{\makebox[0.6cm]{0.029} \, \makebox[0.7cm]{\textcolor{gray}{2,553 spp}}} & \small{\makebox[0.6cm]{0.024} \, \makebox[0.7cm]{\textcolor{gray}{1,093 spp}}} & \small{\makebox[0.6cm]{0.023} \, \makebox[0.7cm]{\textcolor{gray}{1,122 spp}}} & \small{\makebox[0.6cm]{\textbf{0.023}} \, \makebox[0.7cm]{\textcolor{gray}{783 spp}}} & \small{\makebox[0.6cm]{\textbf{0.018}} \, \makebox[0.7cm]{\textcolor{gray}{783 spp}}} & \small{\makebox[0.6cm]{0.036} \, \makebox[0.7cm]{\textcolor{gray}{783 spp}}} \\
  \small{\Torus{}} & \small{\makebox[0.6cm]{0.214} \, \makebox[0.7cm]{\textcolor{gray}{12,108 spp}}} & \small{\makebox[0.6cm]{0.021} \, \makebox[0.7cm]{\textcolor{gray}{9,470 spp}}} & \small{\makebox[0.6cm]{0.021} \, \makebox[0.7cm]{\textcolor{gray}{3,311 spp}}} & \small{\makebox[0.6cm]{0.019} \, \makebox[0.7cm]{\textcolor{gray}{3,211 spp}}} & \small{\makebox[0.6cm]{\textbf{0.016}} \, \makebox[0.7cm]{\textcolor{gray}{3,334 spp}}} & \small{\makebox[0.6cm]{0.015} \, \makebox[0.7cm]{\textcolor{gray}{3,334 spp}}} & \small{\makebox[0.6cm]{\textbf{0.014}} \, \makebox[0.7cm]{\textcolor{gray}{3,334 spp}}} \\
  \small{\VeachDoor{}} & \small{\makebox[0.6cm]{0.532} \, \makebox[0.7cm]{\textcolor{gray}{3,749 spp}}} & \small{\makebox[0.6cm]{0.084} \, \makebox[0.7cm]{\textcolor{gray}{2,773 spp}}} & \small{\makebox[0.6cm]{0.072} \, \makebox[0.7cm]{\textcolor{gray}{561 spp}}} & \small{\makebox[0.6cm]{0.066} \, \makebox[0.7cm]{\textcolor{gray}{535 spp}}} & \small{\makebox[0.6cm]{\textbf{0.047}} \, \makebox[0.7cm]{\textcolor{gray}{682 spp}}} & \small{\makebox[0.6cm]{\textbf{0.028}} \, \makebox[0.7cm]{\textcolor{gray}{682 spp}}} & \small{\makebox[0.6cm]{0.037} \, \makebox[0.7cm]{\textcolor{gray}{682 spp}}} \\
  \small{\VeachLamp{}} & \small{\makebox[0.6cm]{0.532} \, \makebox[0.7cm]{\textcolor{gray}{4,079 spp}}} & \small{\makebox[0.6cm]{0.069} \, \makebox[0.7cm]{\textcolor{gray}{2,204 spp}}} & \small{\makebox[0.6cm]{0.083} \, \makebox[0.7cm]{\textcolor{gray}{499 spp}}} & \small{\makebox[0.6cm]{0.069} \, \makebox[0.7cm]{\textcolor{gray}{471 spp}}} & \small{\makebox[0.6cm]{\textbf{0.057}} \, \makebox[0.7cm]{\textcolor{gray}{655 spp}}} & \small{\makebox[0.6cm]{0.037} \, \makebox[0.7cm]{\textcolor{gray}{655 spp}}} & \small{\makebox[0.6cm]{\textbf{0.025}} \, \makebox[0.7cm]{\textcolor{gray}{655 spp}}} \\
  \bottomrule
\end{tabular*}


==> results-visualizer-figure.tex <==
\setlength{\fboxrule}{1pt}%
\setlength{\insetvsep}{20pt}%
\setlength{\tabcolsep}{1pt}%
\renewcommand{\arraystretch}{0.75}%
\small%
\hspace*{-0.5mm}%
\begin{tabular}{cccccccccccc}
  \multicolumn{4}{c}{\Bedroom{}}&\multicolumn{4}{c}{\Bathroom{}}&\multicolumn{4}{c}{\SpectralBox{}}\\
  \multicolumn{4}{c}{\begin{overpic}[width=0.33\textwidth]{images/fig-references/bedroom-reference-lq.jpg}
\put(77.76041666666667,2.994791666666667){\makebox(0,0){\tikz\draw[red,fill=red] (0,0) circle (0.0033\textwidth);}}
\put(27.500000000000004,50.208333333333336){\makebox(0,0){\tikz\draw[orange,fill=orange] (0,0) circle (0.0033\textwidth);}}
\end{overpic}}&\multicolumn{4}{c}{\begin{overpic}[width=0.33\textwidth]{images/fig-references/bathroom-reference-lq.jpg}
\put(50.06942708333333,4.722239583333335){\makebox(0,0){\tikz\draw[red,fill=red] (0,0) circle (0.0033\textwidth);}}
\put(70.90260416666666,8.402760416666665){\makebox(0,0){\tikz\draw[orange,fill=orange] (0,0) circle (0.0033\textwidth);}}
\end{overpic}}&\multicolumn{4}{c}{\begin{overpic}[width=0.33\textwidth]{images/fig-references/spectral-box-reference-lq.jpg}
\put(60.55572916666667,44.097239583333334){\makebox(0,0){\tikz\draw[red,fill=red] (0,0) circle (0.0033\textwidth);}}
\put(56.944270833333334,18.61109375){\makebox(0,0){\tikz\draw[orange,fill=orange] (0,0) circle (0.0033\textwidth);}}
\end{overpic}}\\
  \color{red}\fbox{\includegraphics[width=0.07583333333333334\textwidth]{images/fig-visualizer/pos-0-bedroom/dump-dist-0-cv-0.jpg}}&\color{red}\fbox{\includegraphics[width=0.07583333333333334\textwidth]{images/fig-visualizer/pos-0-bedroom/dump-dist-0-pdf-0.jpg}}&\color{orange}\fbox{\includegraphics[width=0.07583333333333334\textwidth]{images/fig-visualizer/pos-1-bedroom/dump-dist-0-cv-0.jpg}}&\color{orange}\fbox{\includegraphics[width=0.07583333333333334\textwidth]{images/fig-visualizer/pos-1-bedroom/dump-dist-0-pdf-0.jpg}}&\color{red}\fbox{\includegraphics[width=0.07583333333333334\textwidth]{images/fig-visualizer/pos-0-bathroom/dump-dist-0-cv-0.jpg}}&\color{red}\fbox{\includegraphics[width=0.07583333333333334\textwidth]{images/fig-visualizer/pos-0-bathroom/dump-dist-0-pdf-0.jpg}}&\color{orange}\fbox{\includegraphics[width=0.07583333333333334\textwidth]{images/fig-visualizer/pos-1-bathroom/dump-dist-0-cv-0.jpg}}&\color{orange}\fbox{\includegraphics[width=0.07583333333333334\textwidth]{images/fig-visualizer/pos-1-bathroom/dump-dist-0-pdf-0.jpg}}&\color{red}\fbox{\includegraphics[width=0.07583333333333334\textwidth]{images/fig-visualizer/pos-0-spectral-box/dump-dist-0-cv-0.jpg}}&\color{red}\fbox{\includegraphics[width=0.07583333333333334\textwidth]{images/fig-visualizer/pos-0-spectral-box/dump-dist-0-pdf-0.jpg}}&\color{orange}\fbox{\includegraphics[width=0.07583333333333334\textwidth]{images/fig-visualizer/pos-1-spectral-box/dump-dist-0-cv-0.jpg}}&\color{orange}\fbox{\includegraphics[width=0.07583333333333334\textwidth]{images/fig-visualizer/pos-1-spectral-box/dump-dist-0-pdf-0.jpg}}\\
  CV&PDF&CV&PDF&CV&PDF&CV&PDF&CV&PDF&CV&PDF\\
\end{tabular}


==> teaser-figure-n-tech.tex <==
\setlength{\fboxrule}{15pt}%
\setlength{\insetvsep}{30pt}%
\setlength{\tabcolsep}{-1.5pt}%
\renewcommand{\arraystretch}{1}%
\small%
\begin{tabular}{ccccc}
  & \multicolumn{2}{c}{Unbiased} & \multicolumn{1}{c}{Biased} & \\
  \cmidrule(lr){2-3}
  \cmidrule(lr){4-4}
  \textbf{(d)} Rendering results of the \VeachDoor{} scene & PPG & Ours & +Heuristic & Reference \\
    \setInset{A}{red}{460}{650}{50}{80}%
    \setInset{B}{orange}{1135}{650}{50}{80}%
    \addBeautyCrop{images/fig-references/veach-door-reference-lq.jpg}{0.333}{1920}{1080}{0}{0}{1520}{1080} &
    \addInsets{images/fig-teaser/veach-door-PPG_u.jpg} &
    \addInsets{images/fig-teaser/veach-door-NCV-Ours_u.jpg} &
    \addInsets{images/fig-teaser/veach-door-NCV-Ours_b.jpg} &
    \addInsets{images/fig-references/veach-door-reference.jpg} \\
  \multicolumn{1}{r}{MAPE:} & 0.084 & \textbf{0.047} & \textbf{0.028} & \\
\end{tabular}

